Extreme Nonnegative Quadratics over Stanley Reisner Varieties

We consider the convex geometry of the cone of nonnegative quadratics over Stanley-Reisner varieties. Stanley-Reisner varieties (which are unions of coordinate planes) are amongst the simplest real projective varieties, so this is potentially a starting point that can generalize to more complicated real projective varieties. This subject has some suprising connections to algebraic topology and category theory, which we exploit heavily in our work. These questions are also valuable in applied math, because they directly translate to questions about positive semidefinite (PSD) matrices. In particular, this relates to a long line of work concerning the extent to which it is possible to approximately check that a matrix is PSD by checking that some principle submatrices are PSD, or to check if a partial matrix can be approximately completed to full PSD matrix. We systematize both these practical and theoretical questions using a framework based on algebraic topology, category theory, and convex geometry. As applications of this framework we are able to classify the extreme nonnegative quadratics over many Stanley-Reisner varieties. We plan to follow these structural results with a paper that is more focused on quantitative questions about PSD matrix completion, which have applications in sparse semidefinite programming.

==> tikz_example.tex <==
\begin{tikzpicture}
    % Path Graph
    \node[shape=circle,draw=black] (1) at (1,5) {1};
    \node[shape=circle,draw=black] (3) at (2,5) {2};
    \node[shape=circle,draw=black] (5) at (3,5) {3};
    \node (dots) at (3,6) {$\dots$};
    \node[shape=circle,draw=black] (8) at (2,6) {$n$};
    \node[shape=circle,draw=black] (7) at (1,6) {$1^*$};
    \node[shape=circle,draw=black] (9) at (4,5.5) {$4$};

    \path [-](1) edge node[left] {} (3);
    \path [-](3) edge node[left] {} (5);
    \path [-](8) edge node[left] {} (7);
    \path [-](8) edge node[left] {} (dots);
    \path [-](9) edge node[left] {} (dots);
    \path [-](9) edge node[left] {} (5);

    % Rounded Rectangle
    \draw[rounded corners] (0.5, 6.5) rectangle (1.5, 4.5) {};
    % Arrow
    \draw [->] (1,4.5) -- (1, 3);
    % Cycle Graph

    \node[shape=circle,draw=black] (a1) at (1,2.5) {1};
    \node[shape=circle,draw=black] (a3) at (2,2) {2};
    \node[shape=circle,draw=black] (a5) at (3,2) {3};
    \node (adots) at (3,3) {$\dots$};
    \node[shape=circle,draw=black] (a8) at (2,3) {$n$};
    \node[shape=circle,draw=black] (a9) at (4,2.5) {$4$};

    \path [-](a1) edge node[left] {} (a3);
    \path [-](a3) edge node[left] {} (a5);
    \path [-](a8) edge node[left] {} (a1);
    \path [-](a8) edge node[left] {} (adots);
    \path [-](a9) edge node[left] {} (adots);
    \path [-](a9) edge node[left] {} (a5);
\end{tikzpicture}
